Automatic Completion of Distributed Protocols with Symmetry

A distributed protocol is typically modeled as a set of communicating processes, where each process is described as an extended state machine along with fairness assumptions, and its correctness is specified using safety and liveness requirements. Designing correct distributed protocols is a challenging task. Aimed at simplifying this task, we allow the designer to leave some of the guards and updates to state variables in the description of extended state machines as unknown functions. The protocol completion problem then is to find interpretations for these unknown functions while guaranteeing correctness. In many distributed protocols, process behaviors are naturally symmetric, and thus, synthesized expressions are further required to obey symmetry constraints. Our counterexample-guided synthesis algorithm consists of repeatedly invoking two phases. In the first phase, candidates for unknown expressions are generated using the SMT solver Z3. This phase requires carefully orchestrating constraints to enforce the desired symmetry in read/write accesses. In the second phase, the resulting completed protocol is checked for correctness using a custom-built model checker that handles fairness assumptions, safety and liveness requirements, and exploits symmetry. When model checking fails, our tool examines a set of counterexamples to safety/liveness properties to generate constraints on unknown functions that must be satisfied by subsequent completions. For evaluation, we show that our prototype is able to automatically discover interesting missing details in distributed protocols for mutual exclusion, self stabilization, and cache coherence.

==> figures/elevator_example/elevator_automaton.tex <==
\begin{tikzpicture}[on grid]
  \path
  node[state, initial, initial text={}, initial where=above] (waiting) {$E_0$}
  node[above=1.2cm of waiting] {$\text{floor} \coloneqq 1$}
  node[state, below=3cm of waiting, accepting] (error) {$E_5$} %, label=below:error
  node[state, left=5.5cm of waiting] (up1) {$E_1$}
  node[state, right=5.5cm of waiting] (down1) {$E_3$}
  node[state, left=2.4cm of waiting] (up2) {$E_2$}
  node[state, right=2.4cm of waiting] (down2) {$E_4$}

  (waiting)
  edge[transition, bend right]
  node[transition label] {$\text{floor} < \text{TOP} \land \text{up?} \to$\\$\text{floor}\coloneqq \text{floor}+1$}
  (up1)

  (up1)
  edge[transition]
  node[transition label, below] {at-floor ! floor}
  (up2)

  (up2)
  edge[transition]
  node[transition label, below] {up-ack!}
  (waiting)

  (waiting)
  edge[transition, bend left]
  node[transition label] {$\floor > 1 \land \text{down?} \to$\\ $\text{floor}\coloneqq\text{floor}-1$}
  (down1)

  (down1)
  edge[transition]
  node[transition label, below] {at-floor ! floor}
  (down2)

  (down2)
  edge[transition]
  node[transition label, below] {down-ack!}
  (waiting)

  (waiting)
  edge[transition, bend right]
  node[transition label, left] {$\floor=1 \land \text{down?}$}
  (error)

  (waiting)
  edge[transition, bend left]
  node[transition label, right] {$\floor=\top \land \text{up?}$}
  (error)
  ;
\end{tikzpicture}


==> figures/elevator_example/incomplete_controller_automaton.tex <==
\begin{tikzpicture}[on grid]
  \def\floor{\text{floor}}
  %\def\top{\text{TOP}}
  \def\target{\text{target}}
  \path
  node[state, initial, initial text={}, initial where=left] (waiting) {$C_0$}
  node[state, right=3.8cm of waiting] (working) {$C_1$}
  node[state, above right=2.3cm and 3cm of working] (up) {$C_2$}
  node[state, below right=2.3cm and 3cm of working] (down) {$C_3$}

  (waiting)
  edge[transition]
  node[transition label] {$\text{request?}\to$\\$\text{target}\coloneqq\text{request}$}
  (working)

  (working)
  edge[transition, bend left]
  node[transition label, below] {$g_1(\text{floor}, \text{target})\to$\\ arrive!}
  (waiting)

  (working)
  edge[transition, bend left]
  node[transition label, above left=-.2cm and -.2cm] {$g_2(\text{target}, \text{floor})\to$\\ up!}
  (up)

  (working)
  edge[transition, bend right] node[transition label, below left] {$g_3(\text{target}, \text{floor})\to$\\ down!}
  (down)

  (up)
  edge[transition]
  node[transition label, below right=-.2cm and -.2cm] {$\text{up-ack?}\to$\\$\text{floor}\coloneqq f_1(\text{floor})$}
  (working)

  (down)
  edge[transition]
  node[transition label, above right] {$\text{down-ack?}\to$\\$\text{floor}\coloneqq f_2(\text{floor})$}
  (working)
  ;
\end{tikzpicture}


==> figures/elevator_example/liveness_monitor.tex <==
\begin{tikzpicture}[on grid, node distance=3cm]
  \def\looseness{10}
  \path
  node[state, initial, initial text={}, initial where=left] (initial) {$L_0$}
  node[state, right=of initial, accepting] (requested) {$L_1$} % , label=270:accept
  node[state, right=of requested] (granted) {$L_2$}

  (initial)
  edge[transition]
  node[transition label] {request?}
  (requested)

  (initial)
  edge[transition, loop above, looseness=\looseness]
  node[transition label] {request?}
  (initial)

  (initial)
  edge[transition, loop below, looseness=\looseness]
  node[transition label, below] {arrive?}
  (initial)

  (requested)
  edge[transition, loop above, looseness=\looseness]
  node[transition label] {request?}
  (requested)

  (requested)
  edge[transition]
  node[transition label] {arrive?}
  (granted)

  (granted)
  edge[transition, loop above, looseness=\looseness]
  node[transition label] {request?}
  (granted)

  (granted)
  edge[transition, loop below, looseness=\looseness]
  node[transition label, below] {arrive?}
  (granted)
  ;
\end{tikzpicture}


==> figures/elevator_example/safety_monitor.tex <==
\begin{tikzpicture}[on grid, node distance=5cm]
  \path
  node[state, initial, initial text={}, initial where=left] (initial) {$S_0$}
  node[state, right=7cm of initial] (requested) {$S_1$}
  node[state, accepting] at ($(initial)!.5!(requested) - (0, 4)$) (error) {$S_2$} % , label=270:error
  node[align=center, above left=1cm and .3cm of initial]
  {\trupdate{safety-floor := 1;}\\\trupdate{safety-target := 1}}

  (initial)
  edge[transition]
  node[transition label] {$\text{request?} \to$\\$\text{safety-target} \coloneqq \text{request}$}
  (requested)

  (initial)
  edge[transition, bend right]
  node[transition label, left] {arrive?}
  (error)

  (requested)
  edge[transition, loop above, looseness=10]
  node[transition label, above=0cm] {$\text{at-floor?}\to$\\$\text{safety-floor}\coloneqq\text{at-floor}$}
  (requested)

  (requested)
  edge[transition, bend left]
  node[transition label, below left=0cm and -1.5cm] {$\text{safety-floor} = \text{safety-target} \land$\\$\text{arrive?}$}
  (initial)

  (requested)
  edge[transition]
  node[transition label, below left=.2cm and .5cm] {$\text{request?}$}
  (error)

  (requested)
  edge[transition, bend left]
  node[transition label, below right=.6cm and -.7cm] {$\text{safety-floor} \neq \text{safety-target} \land$\\$\text{arrive?}$}
  (error)
  ;
\end{tikzpicture}


==> figures/elevator_example/user_automaton.tex <==
\begin{tikzpicture}[on grid]
  \path
  node[state, initial, initial text={}] (initial) {$U_0$}
  node[state, right=4cm of initial] (waiting) {$U_1$}
  node at ($(initial)!.5!(waiting)$) {$\vdots$}

  (initial)
  edge[transition, bend left] node[transition label]
  {
    request ! 1
  }
  (waiting)

  (initial)
  edge[transition, bend right] node[transition label, below]
  {
    request ! TOP
  }
  (waiting)

  (waiting)
  edge[transition, out=90, in=90, looseness=1.3] node[transition label] {arrive?}
  (initial)
  ;
\end{tikzpicture}


==> figures/leader_election/leader_monitor.tex <==
\begin{tikzpicture}[on grid]
  \def\angle{70}

  \path
  node[state, initial, initial text={}] (s0) {$S_0$}
  node[state, right=4cm of s0] (s1) {$S_1$}
  node[state, right=4cm of s1] (s2) {$S_2$}
  node[state, right=3cm of s2, accepting] (s3) {$S_3$}

  (s0)
  edge[transition]
  node[transition label]
  {$\text{leader}_\text{1}? \to$\\$\text{leader-id} \coloneqq \text{leader}_\text{1}$}
  (s1)

  (s0)
  edge[transition, out=80, in=100]
  node[transition label]
  {$\text{leader}_\text{N}? \to$\\$\text{leader-id} \coloneqq \text{leader}_\text{N}$}
  (s1)

  node[at={($(s0)!.5!(s1)+(0, 1.25)$)}] {$\vdots$}

  (s1)
  edge[transition]
  node[transition label, above]
  {$\text{leader-id} = \text{MAX-ID}$}
  (s2)

  (s1)
  edge[transition, out=80, in=100]
  node[transition label, above]
  {$\text{leader-id} \neq \text{MAX-ID}$}
  (s3)

  (s2)
  edge[transition]
  node[transition label]
  {$\text{leader}_\text{1}?$}
  (s3)

  (s2)
  edge[transition, out=70, in=110]
  node[transition label]
  {$\text{leader}_\text{N}?$}
  (s3)

  node[at={($(s2)!.5!(s3)+(0, 0.9)$)}] {$\vdots$}
  ;
\end{tikzpicture}


==> figures/leader_election/liveness_monitor.tex <==
\begin{tikzpicture}[on grid]
  \def\angle{70}
  \path
  node[state, accepting, initial, initial text={}] (s0) {$S_0$}
  node[state, right=4cm of s0] (s1) {$S_1$}

  (s0)
  edge[transition]
  node[transition label]
  {$\text{leader}_\text{1}?$}
  (s1)

  (s0)
  edge[transition, out=80, in=100]
  node[transition label]
  {$\text{leader}_\text{N}?$}
  (s1)

  node[at={($(s0)!.5!(s1)+(0, 1.2)$)}] {$\vdots$}

  (s1)
  edge[transition, out=-70, in=250, looseness=5]
  node[transition label, below]
  {$\text{leader}_\text{1}?$}
  (s1)

  (s1)
  edge[transition, out=-40, in=220, looseness=12]
  node[transition label, below]
  {$\text{leader}_\text{N}?$}
  (s1)

  node[at={($(s1)-(0, 1.3)$)}] {$\vdots$}

  ;
\end{tikzpicture}


==> figures/leader_election/process.tex <==
\begin{tikzpicture}[on grid]
  \def\angle{70}
  \path
  node[state, initial above, initial text={}] (p0) {$P_0$}
  node[state, left=2.5cm of p0] (p1) {$P_1$}
  node[state, right=4cm of p0] (p2) {$P_2$}
  node[state, right=4cm of p2] (p3) {$P_3$}

  (p0)
  edge[transition]
  node[transition label]
  {$\text{elect} ?$}
  (p1)

  (p1)
  edge[transition, out=360-\angle, in=180+\angle]
  node[transition label, below]
  {$\text{right} ! \text{id}$}
  (p0)

  (p0)
  edge[transition]
  node[transition label, above]
  {$\text{left} ? \to$\\$\text{input-id} \coloneqq \text{left}$}
  (p2)

  (p2)
  edge[transition, out=180-\angle, in=\angle]
  node[transition label, above]
  {$\text{input-id} > \text{id} \to$\\$\text{right} ! \text{input-id}$}
  (p0)

  (p2)
  edge[transition, out=180+\angle, in=360-\angle]
  node[transition label, below]
  {$\text{input-id} < \text{id} \to$\\$\text{right} ! \text{id}$}
  (p0)

  (p2)
  edge[transition]
  node[transition label, above]
  {$\text{input-id} = \text{id} \to$\\$\text{leader} ! \text{id}$}
  (p3)
  ;
\end{tikzpicture}


==> figures/msi/msi_scenario_header.tex <==
\usetikzlibrary{arrows}
\tikzstyle{lane} = [draw, loosely dotted, ->, >=latex, line width=1.3]
\tikzstyle{message} = [draw, ->, >=latex, line width=2]
\tikzstyle{intmsg} = [draw, ->, >=latex, line width=2]
\tikzstyle{tentmessage} = [draw, dashed, ->, >=latex, line width=2]
\tikzstyle{message node} = [sloped, align=center, above, pos=.5,font=\small]
\tikzstyle{command node} = [align=center,font=\small]
\tikzstyle{lane label} = [align=center,font=\small]
\tikzstyle{figure letter} = [font={\LARGE\bf}, below=.2cm]


==> figures/msi/scenarios.tex <==
%!TEX root = ../../cav15.tex

\tikzstyle{lane} = [draw, loosely dotted, ->, >=latex, line width=1.3]
\tikzstyle{message} = [draw, ->, >=latex, line width=2]
\tikzstyle{message node} = [sloped, align=center, above, pos=.5]
\tikzstyle{command node} = [align=center]
\tikzstyle{lane label} = [align=center]
\tikzstyle{figure letter} = [font={\LARGE\bf}, below=.2cm]


==> figures/peterson/complete_process_0.tex <==
%!TEX root = ../../cav15.tex

\begin{tikzpicture}
  \path
  node[state, initial, initial text={}] (L1) {$L_1$}
  node[state, right=2.1cm of L1] (L2) {$L_2$}
  node[state, right=1.5cm of L2] (L3) {$L_3$}
  node[state, below=.4cm of L2] (Critical) {$L_4$}
  node[below=.03cm of Critical] {Critical section}
  ;
  \path
  (L1)
  edge[transition]
  node[transition label]
  {
  $\text{request}_\texttt{P0}!$\\
  $\text{flag}[\texttt{P0}] \coloneqq \true$
  }
  (L2)
  (L2)
  edge[transition]
  node[transition label]
  {
  $\text{turn} \coloneqq \texttt{P1}$
  }
  (L3)
  (L3)
  edge[transition, out=70, in=110, looseness=6]
  node[transition label]
  {
  $\text{flag}[\texttt{P1}] \land \text{turn} = \texttt{P1}$\\
  $\text{waiting}_\texttt{P0}!$
  }
  (L3)
  (L3)
  edge[transition]
  node[transition label, below right=.05cm and -.4cm]
  {$\lnot \text{flag}[\texttt{P1}] \lor \text{turn} = \texttt{P0}$\\
  $\text{critical}_\texttt{P0}!$}
  (Critical)
  (Critical)
  edge[transition]%, out=230, in=-50]
  node[transition label, below left=.1cm and -.6cm]
  {
  $\text{flag}[\texttt{P0}]\coloneqq \false$
  }
  (L1)
  ;
\end{tikzpicture}


==> figures/peterson/complete_process_1.tex <==
%!TEX root = ../../cav15.tex

\begin{tikzpicture}
  \path
  node[state, initial, initial text={}] (L1) {$L_1$}
  node[state, right=2.1cm of L1] (L2) {$L_2$}
  node[state, right=1.5cm of L2] (L3) {$L_3$}
  node[state, below=.4cm of L2] (Critical) {$L_4$}
  node[below=.03cm of Critical] {Critical section}
  ;
  \path
  (L1)
  edge[transition]
  node[transition label]
  {
  $\text{request}_\texttt{P1}!$\\
  $\text{flag}[\texttt{P1}] \coloneqq \true$
  }
  (L2)
  (L2)
  edge[transition]
  node[transition label]
  {
  $\text{turn} \coloneqq \texttt{P0}$
  }
  (L3)
  (L3)
  edge[transition, out=70, in=110, looseness=6]
  node[transition label]
  {
  $\text{flag}[\texttt{P0}] \land \text{turn} = \texttt{P0}$\\
  $\text{waiting}_\texttt{P1}!$
  }
  (L3)
  (L3)
  edge[transition]
  node[transition label, below right=.05cm and -.4cm]
  {$\lnot \text{flag}[\texttt{P0}] \lor \text{turn} = \texttt{P1}$\\
  $\text{critical}_\texttt{P1}!$}
  (Critical)
  (Critical)
  edge[transition]%, out=230, in=-50]
  node[transition label, below left=.1cm and -.6cm]
  {
  $\text{flag}[\texttt{P1}]\coloneqq \false$
  }
  (L1)
  ;
\end{tikzpicture}

